On the Cryptographic Hardness of Learning Single Periodic Neurons

We show a simple reduction which demonstrates the cryptographic hardness of learning a single periodic neuron over isotropic Gaussian distributions in the presence of noise. More precisely, our reduction shows that any polynomial-time algorithm (not necessarily gradient-based) for learning such functions under small noise implies a polynomial-time quantum algorithm for solving worst-case lattice problems, whose hardness form the foundation of lattice-based cryptography. Our core hard family of functions, which are well-approximated by one-layer neural networks, take the general form of a univariate periodic function applied to an affine projection of the data. These functions have appeared in previous seminal works which demonstrate their hardness against gradient-based (Shamir'18), and Statistical Query (SQ) algorithms (Song et al.'17). We show that if (polynomially) small noise is added to the labels, the intractability of learning these functions applies to all polynomial-time algorithms, beyond gradient-based and SQ algorithms, under the aforementioned cryptographic assumptions. Moreover, we demonstrate the necessity of noise in the hardness result by designing a polynomial-time algorithm for learning certain families of such functions under exponentially small adversarial noise. Our proposed algorithm is not a gradient-based or an SQ algorithm, but is rather based on the celebrated Lenstra-Lenstra-Lov\'asz (LLL) lattice basis reduction algorithm. Furthermore, in the absence of noise, this algorithm can be directly applied to solve CLWE detection (Bruna et al.'21) and phase retrieval with an optimal sample complexity of $d+1$ samples. In the former case, this improves upon the quadratic-in-$d$ sample complexity required in (Bruna et al.'21).

==> Hardness of Learning (arxiv)/custom_commands.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath}
\usepackage{amstext}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{bbm}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[ruled,vlined]{algorithm2e}

%%%%%%%%% BIBLATEX %%%%%%%%%
\usepackage[
backend=biber,
style=alphabetic,
citestyle=alphabetic,
giveninits=false,
maxnames=99,
date=year
]{biblatex}
\AtEveryBibitem{%
\ifentrytype{article}{
    \clearfield{url}%
    \clearfield{urldate}%
    \clearfield{eprint}%
    \clearfield{review}%
    \clearfield{location}%
    \clearfield{address}%
    \clearfield{issn}%
    \clearfield{isbn}%
    \clearfield{doi}%
    \clearfield{series}%%
    }{}%
\ifentrytype{inproceedings}{
    \clearlist{publisher}%
    \clearlist{location}%
    \clearfield{url}%
    \clearfield{urldate}%
    \clearfield{issn}%
    \clearfield{isbn}%
    \clearfield{doi}%
    \clearfield{series}%%
}{}%
\ifentrytype{book}{
    \clearfield{url}%
    \clearfield{urldate}%
    \clearfield{review}%
    \clearfield{location}%
    \clearfield{address}%
    \clearfield{issn}%
    \clearfield{isbn}%
    \clearfield{doi}%
    \clearfield{series}%%
}{}%
\ifentrytype{inbook}{
    \clearfield{url}%
    \clearfield{urldate}%
    \clearfield{review}%
    \clearfield{location}%
    \clearfield{address}%
    \clearfield{issn}%
    \clearfield{isbn}%
    \clearfield{doi}%
    \clearfield{eprint}%
    \clearfield{series}%%
}{}%
\ifentrytype{incollection}{
    \clearfield{url}%
    \clearfield{urldate}%
    \clearfield{review}%
    \clearfield{location}%
    \clearfield{address}%
    \clearfield{issn}%
    \clearfield{isbn}%
    \clearfield{doi}%
    \clearfield{series}%%
}{}
}

\DeclareFieldFormat[inproceedings]{title}{#1} 
\DeclareFieldFormat[article]{title}{#1}
\DeclareFieldFormat[inbook]{title}{#1}
\DeclareFieldFormat[misc]{title}{#1}
\DeclareFieldFormat[article]{year}{#1}
\DeclareFieldFormat[book]{title}{#1}

\renewbibmacro{in:}{}
\renewcommand{\multicitedelim}{\addcomma\space} % MJ: add comma for multiple citations.
\renewbibmacro*{volume+number+eid}{%
  \printfield{volume}
  \setunit{\addcolon\space}%
  \printfield{number}%
  \printfield{eid}}


% \AtEveryBibitem{
%     \clearfield{url}
%     \clearfield{urldate}
%     \clearfield{review}
%     \clearfield{location}
%     \clearfield{doi}
%     \clearfield{series}
%     \clearfield{publisher}
%     \clearfield{issn}
%     \clearfield{isbn}
%     \clearfield{address}
% }
\addbibresource{reference.bib}
\addbibresource{group.bib}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{question}[theorem]{Question}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{example}[theorem]{Example}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{fact}[theorem]{Fact}

%\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}

\newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\PP}{\mathbb{P}}
% \newcommand{\SS}{\mathbb{S}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\sA}{\mathcal{A}}
\newcommand{\sB}{\mathcal{B}}
\newcommand{\sC}{\mathcal{C}}
\newcommand{\sD}{\mathcal{D}}
\newcommand{\sF}{\mathcal{F}}
\newcommand{\sH}{\mathcal{H}}
\newcommand{\sK}{\mathcal{K}}
\newcommand{\sN}{\mathcal{N}}
\newcommand{\sP}{\mathcal{P}}
\newcommand{\sT}{\mathcal{T}}
\newcommand{\sS}{\mathcal{S}}

\newcommand{\eps}{\epsilon}

\DeclareMathOperator*{\EE}{\mathbb{E}}
\DeclareMathOperator*{\prob}{\mathbb{P}}
\newcommand{\Var}{\mathop{\mathrm{Var}}}
\newcommand{\one}{\mathop{\mathbbm{1}}}
\newcommand{\One}{\mathbbm{1}}
\newcommand{\symd}{\bigtriangleup}

\newcommand{\PGW}{\mathrm{PGW}}
\newcommand{\ER}{Erd\H{o}s--R\'{e}nyi }
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\Pois}{\mathrm{Pois}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\Adv}{\mathsf{Adv}}
\newcommand{\poly}{\mathsf{poly}}
\newcommand{\negl}{\mathsf{negl}}
\newcommand{\SVP}{\ensuremath{\mathrm{SVP}}}
\newcommand{\CVP}{\ensuremath{\mathrm{CVP}}}

\newcommand{\bw}{\bm w}
\newcommand{\bx}{\bm x}
\newcommand{\by}{\bm y}
\newcommand{\bY}{\bm Y}

\newcommand{\clwe}{\mathrm{CLWE}}

\newcommand{\JB}[1]{\textcolor{cyan}{joan: #1}}
%%% AD-HOC NEW COMMANDS
\renewcommand{\Pr}{\mathbb{P}}

==> Hardness of Learning (arxiv)/itsample.tex <==
\section{Optimality of \texorpdfstring{$d+1$}{d+1} samples for exact recovery under norm priors}
\label{optim_sample_app}

In this appendix, we argue that $d+1$ samples are necessary in order to obtain exact recovery with probability $1-\exp(-\Omega(d))$, 
irrespective of any estimation procedure. 
Since our upper bound holds for arbitrary $w/\|w\|_2 \in {S}^{d-1},$ and arbitrary $1 \leq \gamma =\|w\|_2=\mathrm{poly}(d)$, 
it suffices to prove a lower bound for \emph{some} distributional assumption on $\gamma$ and $w/\|w\|_2$ which respects these constraints. 
Hence, for our lower bound, we assume a uniform prior on the direction $w/\|w\|_2 \in S^{d-1}$, and assume that $\gamma=\|w\|_2>0$ is distributed independently of $w$ according to a probability density $q_\gamma$ which satisfies the following assumption.
\begin{assumption}
\label{assump:basicapp} For some $B>\sqrt{2}$ and $C>0$, the function $q_{\gamma}: \mathbb{R} \rightarrow [0,\infty)$ satisfies that
$q_{\gamma}(t) t^{-d+1}$ is non-increasing for $t \in [1, B]$, and  $\int_{\sqrt{2}}^B q_{\gamma}(t) dt \geq C$. 
\end{assumption}

We now state our lower bound, restating Theorem \ref{thm:IToptim} for convenience.
\begin{theorem}
\label{thm:IToptimapp}
Consider $d\geq 2$ samples $\{(x_i, y_i=|\inner{x_i, w}|) \}_{i=1\ldots d}$, in which the $x_i$'s are drawn i.i.d. from $N(0,I_d)$, and $w$ is drawn from two independent variables: $w/\|w\|$ uniformly distributed in $S^{d-1}$ and $\|w\|$ distributed with density satisfying Assumption \ref{assump:basicapp}. Let $\mathcal{A}$ be any estimation procedure (deterministic or randomized) that takes as input $\{(x_i, y_i)\}_{i=1,\ldots,d}$ and outputs $w' \in \mathbb{R}^d$. Then with probability $\omega(d^{-2})$ it holds $w' \not \in \{-w,w\}.$
\end{theorem}

\begin{proof}
The key idea of the proof will be to establish that with probability $\omega(d^{-2})$ over the draws of the data $\{ x_i \}_{i=1,\ldots,d}$ and the hidden vector $w$, the following event occurs: There exist a pair of antipodal solutions $\{-w',w'\}$ different from $\pm w$, such that the posterior probability measure $p(\tilde{w}~|~ \{(x_i, y_i)\}_{i=1,\ldots,d})$ over any possible hidden vector $\tilde{w} \in \mathbb{R}^d$ 
satisfies $p( \{-w',w'\}~|~ \{(x_i, y_i)\}) \geq p( \{- w, w \}| ~|~\{(x_i, y_i)\})$. In this event, the MAP estimator will thus fail to exactly recover $\{- {w}, {w} \}$ at least with probability $1/2$ (over the randomness of the algorithm). Finally, using the  optimality of the Maximum-a-Posteriori Bayes estimator in minimizing the probability of error, the result follows. 


Let $X=(x_i)_{i=1\ldots d} \in \mathbb{R}^{d \times d}$, be the matrix where for $i=1,\ldots,d$ with $i$-th \emph{row}
equal to $x_i^\top$, and $X^{-1}$ its inverse (which exists with probability $1$ since the determinant of a squared matrix with i.i.d. Gaussian entries is non-zero almost surely \cite{caron2005zero}). Furthermore, let $y = (y_i)_{i=1\ldots d} \in \mathbb{R}^d$ the vector of the labels.
Let us introduce binary variables $\varepsilon \in \{-1,1\}^d$, and the associated matrix
\begin{align*}
    A_\varepsilon := X^{-1} \mathrm{diag}(\varepsilon) X, \;.
\end{align*}
where by $\mathrm{diag}(\varepsilon)$ we refer to the $d \times d$ diagonal matrix with the vector $\varepsilon$ on the diagonal.

We say that a $w' \in \mathbb{R}^d$ is a feasible solution if for all $i=1,\ldots, d$ it holds that $|\inner{ x_i, w'} | = y_i$. Notice that if $w'$ is a feasible solution, then for any $\varepsilon \in \{-1,1\}^d$, 
$A_\varepsilon w'$ is also a feasible solution. This follows since for each $i=1,\ldots,d$ it holds by definition $x_i^\top X^{-1}=e_i^{\top}$, where $e_i$ is the $i$-th standard basis vector, and therefore $x_i^\top A_{\epsilon}=\varepsilon_i x_i^\top$. Hence we have
\begin{align*}
|x_i^\top A_\varepsilon w'|= | \varepsilon_i x_i^\top w' | = y_i\;.
\end{align*} 
On the other hand, if $w'$ is a feasible solution, then there exists $\varepsilon \in \{-1,1\}^d,$ for which for all $i=1,\ldots, d$, it holds $\inner{x_i, w'} = \varepsilon_i y_i$. Therefore, using the definition of $y_i$ and the already established properties of $A_{\varepsilon}$,
\begin{align*} 
\inner{x_i, w'} = \varepsilon_i y_i= x_i^\top \varepsilon_i {w} =x_i^\top A_{\varepsilon}w \;.
\end{align*}

Hence, $X(w'-A_{\varepsilon}{w})=0$. As $X$ is invertible almost surely, we conclude that $w'=A_{\varepsilon}{w}.$ Combining the above, we conclude that the set of feasible solutions is almost surely the set $$\mathcal{B}_{{w}}=\{A_{\varepsilon}{w} | \varepsilon \in \{-1,1\}^d\}.$$ Of course, this set includes ${w}$ when $\varepsilon=\mathbf{1}$ is the all-one vector, and $-{w}$ when $\varepsilon=-\mathbf{1}$ is the all-minus-one vector. Furthermore, from the almost sure linear independence of all $x_i, i=1,\ldots, d+1$, and that $w$ is drawn independent of $X$, we conclude that for all $\varepsilon \not \in \{-\mathbf{1},\mathbf{1}\}$ it holds almost surely that $A_{\varepsilon}{w} \not \in \{-{w},{w}\}.$

Now consider the joint density of the setup in this notation (where we recall that $\tilde{w} \in \mathbb{R}^d$ denotes the generic vector to be recovered, while $w$ is the actual draw of the prior), which decomposes as
\begin{align*} p(X, \tilde{w}, y) = p_X(X) \cdot p_{\tilde{w}}(\tilde{w}) \cdot p( y~|~X, \tilde{w})~, X \in \mathbb{R}^{d \times d}, \tilde{w} \in \mathbb{R}^d, y \in \mathbb{R}^d~.\end{align*}
Notice that since we work under the noiseless assumption it holds 
$p(y~|~X, \tilde{w}) = \delta\left(y- |X \tilde{w}|\right)$,
where by a slight abuse of notation for a vector $v \in \mathbb{R}^d$ we denote by $|v| \in \mathbb{R}^d$ the vector with elements $|v_i|, i=1,\ldots,d$.
Further recall that in this notation we sample a hidden ${w} \sim p_{\tilde{w}}$ and independently a matrix  $X \sim p_X$. We observe the vector of labels $y = |X w|$ and $X$. The posterior probability $p( \tilde{w} ~|~X, y)$ is therefore 
\begin{align}
\label{eq:posteriorprob}
p( \tilde{w} ~|~X, y) = \frac{p(X, \tilde{w}, y)}{p(X, y)} \propto p_{\tilde{w}}(\tilde{w}) \cdot p( y~|~X, \tilde{w})~.    
\end{align}
From our previous argument, we know that this posterior distribution is  necessarily supported in the set $\mathcal{B}_{{w}}$ of $2^d$ points of the form $(X^{-1} \cdot \mathrm{diag}(\varepsilon)) y$ for any $\varepsilon \in \{-1,1\}^d$, which include ${w}$. Denoting by $\delta(\tilde{w})$ the Dirac unit mass at $\tilde{w}$, we have
\begin{align}
\label{eq:bubu}
p( \tilde{w} ~|~X, y) = \frac{1}{Z}\sum_{w' \in \mathcal{B}_{{w}}} \alpha_{X, y}(w') \delta(\tilde{w} - w')~,    
\end{align}
for some normalizing constant $Z$ and some coefficients $\alpha_{X, y}(\varepsilon)$ that we now determine. 
We evaluate the posterior distribution over $\tilde{w}$ from (\ref{eq:posteriorprob}) using the coarea formula~\cite{maly2003co}: Given an arbitrary test function $\phi \in C^\infty_c(\mathbb{R}^d)$, and $F: \mathbb{R}^d \to \mathbb{R}^d$ defined as $F(u):= | X u |$, we have
\begin{eqnarray}
Z \int_{\mathbb{R}^d} p( \tilde{w}~|~X, y) \phi(\tilde{w}) d\tilde{w} &=& \int_{\mathbb{R}^d} p_{\tilde{w}}( \tilde{w}) \delta( y - F(\tilde{w})) \phi(\tilde{w}) d\tilde{w} \\ 
&=& \int_{\mathbb{R}^d} \left(\int_{ F^{-1}(z) } \delta(y - z) p_{\tilde{w}}( u) \phi(u) |DF(u)|^{-1} d\mathcal{H}_0(u) \right) dz \\
&=& \int_{\mathbb{R}^d} \delta(y- z) \left(\int_{ \mathcal{B}_z } p_{\tilde{w}}( u) \phi(u) |DF(u)|^{-1} d\mathcal{H}_0(u) \right) dz \\
&=& \sum_{w' \in \mathcal{B}_w} p_{\tilde{w}}( w' ) \phi( w' ) |\mathrm{det}(X)|^{-1} ~,
\end{eqnarray}
where $d\mathcal{H}_0$ is the $0$-th dimensional Hausdorff measure. 
From (\ref{eq:bubu}) we also have that 
\begin{align*}
 \int_{\mathbb{R}^d} p( \tilde{w}~|~X, y) \phi(\tilde{w}) d\tilde{w} = \sum_{w' \in \mathcal{B}_w} \alpha_{X,y}(w') \phi( w')\;,
\end{align*}
hence we deduce that the weights in (\ref{eq:bubu}) satisfy
\begin{align*}
\forall~\varepsilon~,~    \alpha_{X, y}(X^{-1} \cdot \mathrm{diag}(\varepsilon) y) = p_{\tilde{w}}( X^{-1} \cdot \mathrm{diag}(\varepsilon) y ) |\mathrm{det}(X)|^{-1}~.
\end{align*}
By plugging $y = |X {w}| = \mathrm{diag}(\varepsilon^*) X {w}$ for the sign coefficients $\varepsilon^*_i = \mathrm{sign}( \inner{x_i, w} )$, and recalling the definition of $A_\varepsilon$, we conclude that the posterior distribution over the hidden vector $\tilde{w}$ satisfies almost surely

\begin{align*} 
p( \tilde{w} ~|~X, y)= \left\{
\begin{array}{ll}
      \frac{1}{{Z}} p_{\tilde{w}}(\tilde{w}) & \tilde{w} \in \mathcal{B}_{{w}} \\
      0 & \tilde{w} \not \in \mathcal{B}_{{w}}\\
\end{array} 
\right.
\end{align*}
where ${Z}:=\sum_{\tilde{w} \in \mathcal{B}_{{w}}} p_{\tilde{w}}(\tilde{w})$.

Now to prove the desired result, based on the folklore optimality of the Maximum-A-Posteriori (MAP) estimator in minimizing probability of failure of exact recovery (see Lemma \ref{lem:mapoptim} for completeness) it suffices to prove that with probability $\omega(d^{-2})$ there exists  ${w}' \in \mathcal{B}_{{w}} \setminus \{-{w}, {w}\}$ such that 
\begin{align}
\label{eq:b00cond}
p_{\tilde{w}}({w}')\geq p_{\tilde{w}}({w})~.    
\end{align}
Indeed, recall that since $p_{\tilde{w}}$ is rotationally invariant, we have $p_{\tilde{w}}(\tilde{w}) = p_{\tilde{w}}(-\tilde{w})$ for any $\tilde{w}$, therefore (\ref{eq:b00cond}) immediately implies $p_{\tilde{w}}(\pm {w}')\geq p_{\tilde{w}}(\pm {w}).$ Hence, the  MAP estimator (and therefore any estimator) fails to exactly recover an element of $\{w,-w\}$ with probability  $\omega(d^{-2})$, as we wanted.


Now, using a standard change of variables to spherical coordinates, for all $\tilde{w} \in \mathbb{R}^d$ the density of the prior equal to
$p_{\tilde{w}}(\tilde{w}) = q_\gamma(\| \tilde{w}\|_2 ) \| \tilde{w}\|_2^{-d+1}$.  In particular, based on Assumption~\ref{assump:basic} it suffices to prove that with probability $\omega(d^{-2})$ there exists a ${w}'  \in \mathcal{B}_{{w}} \setminus \{-{w}, {w}\}$ such that $1 \leq \|{w}'\|_2<\|{w}\|_2,$ or equivalently there exists  $\varepsilon \in \{-1,1\}^d \setminus \{- \mathbf{1}, \mathbf{1}\}$ such that
\begin{align}
\label{eq:mainidea}
 1 \leq \| A_\varepsilon {w} \|_2< \|{w} \|_2 ~.   
\end{align}

We establish (\ref{eq:mainidea}) by actually studying only one such $\varepsilon,$ potentially the simplest choice, which we call  $\varepsilon^{(1)}$ where $\varepsilon^{(1)}_1 = -1$ and $\varepsilon^{(1)}_j = +1$ for $j=2,\ldots,d$. This is accomplished by the following key lemma:
\begin{lemma}
\label{lem:ITlem_new}
Suppose $X \in \mathbb{R}^{d \times d}$ has i.i.d. $N(0,I_d)$ entries, and ${w}$ is drawn independently of $X$, such that $w/\|w\|_2$ is drawn from the uniform measure of $S^{d-1}$ and its norm $\|w\|_2$ is independent of $w/\|w\|_2$ and distributed according to a density $q_{\gamma}$ satisfying Assumption~\eqref{assump:basic}. Set also $A_{\varepsilon^{(1)}}=X^{-1}\mathrm{diag}(\varepsilon^{(1)})X$. Then with probability greater than $ \omega(d^{-2})$, it holds
\begin{eqnarray}
1  \leq   \| A_{\varepsilon^{(1)}} {w} \|_2 < \|{w}\|_2 ~. \label{eq:ITpart1} 
\end{eqnarray}
\end{lemma}
This lemma thus proves (\ref{eq:mainidea}) and the failure of the MAP estimator with probability $\omega(d^{-2})$. 

 We conclude the proof by formally stating and using the optimality of the MAP estimator in terms of minimizing the error probability, by relating it to a standard error correcting setup. From our previous argument, we can reduce ourselves to decoders that operate in the discrete set $\mathcal{B}_{{w}}$, since any $\tilde{w}$ outside this set will be different from $\pm {w}$ almost surely. 
\begin{lemma}
\label{lem:mapoptim}
Suppose $\mathcal{X}$ is a discrete set, and let ${x}^* \in \mathcal{X}$ be an element to be recovered, with posterior distribution $p(x | y )$, $x\in \mathcal{X}$, after having observed the output $y=g(x^*)$. Then, any estimator producing $\hat{x}=\hat{x}(y)$ will incur in an error probability $\mathbb{P}(\hat{x} \neq x^*)$ at least $1 - \max_x p(x|y)$, with equality if $\hat{x}$ is the Maximum-A-Posterior (MAP) estimator which outputs $\arg \max_x p(x|y).$
\end{lemma}
We apply the Lemma \ref{lem:mapoptim} for $\mathcal{X}$ containing all the pairs of antipodal elements of $\mathcal{B}_w$, that is $\mathcal{X}=\{ \{w',-w'\} : w' \in \mathcal{B}_{w}\}$ and $x^*=\{w,-w\}.$ As we have established that the MAP estimator fails to exactly recover $x^*$ with probability $\omega(d^{-2})$ this completes the proof.

\end{proof}
\subsection{Proof of Lemma \ref{lem:ITlem_new}}
\begin{proof}

If $e_1$ denotes the first standard basis vector, observe that by elementary algebra,
\begin{align}
\label{eq:basic0}
A_{\varepsilon^{(1)}} = X^{-1} \left( I_d - 2 e_1 e_1^\top \right) X = I_d - 2 \tilde{x}_1 x_1 ~,    
\end{align}
where $x_1^\top$ is the first row of $X$ and $\tilde{x}_1$ is the first column of $X^{-1}$. 

We need a spectral decomposition of matrices of the form $A = I_d - 2 u v^\top$, which is provided in the following lemma:
\begin{lemma}
\label{lem:basiclem}
Let $\eta \in \mathbb{R}$ and $A = I_d - 2 \eta u v^\top \in \mathbb{R}^{d \times d}$, with $\|u \|_2 = \|v \|_2=1$, and $\alpha = \inner{u, v}$. 
Then 
$A^\top A$ has the eigenvalue $1$ with multiplicity $d-2$, 
and two additional eigenvalues $\lambda_{1}, \lambda_2$ with multiplicity $1$ given by
\begin{align}
\label{eq:basic1}
\lambda_{1} = 1 + 2\eta \left( \eta - \alpha - \sqrt{\eta^2 + 1 - 2\eta \alpha} \right) ~,~ \lambda_{2} = 1 + 2\eta \left( \eta - \alpha + \sqrt{\eta^2 + 1 - 2\eta \alpha} \right) ~.    
\end{align}
In particular, $\lambda_{\mathrm{min}}(A^\top A) = \lambda_1 < 1$ and $\lambda_{\mathrm{max}}(A^\top A) = \lambda_2 >1$ whenever $\eta > 0$ and $|\alpha| <1 $.
\end{lemma}

From (\ref{eq:basic0}), we now apply Lemma \ref{lem:basiclem}. By noting that $\inner{x_1, \tilde{x}_1} = 1$ since $X X^{-1} = I_d$, note that the lemma applies for $A_{\varepsilon^{(1)}}$ with parameters
\begin{align*}
\alpha = \left\langle \frac{x_1}{\|x_1\|_2}, \frac{\tilde{x}_1}{\|\tilde{x}_1\|_2} \right\rangle =  \frac{1}{\| x_1 \|_2 \cdot \| \tilde{x}_1 \|_2}~\text{, and } \eta = \| x_1 \|_2 \cdot \| \tilde{x}_1 \|_2\;.\end{align*} 
Since $|\alpha| \in (0,1]$ by Cauchy-Schwarz and
and $\alpha \eta=1$, it follows that $\eta \geq 1$ and the eigenvalues of $A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}}$ are
$\left(\lambda_{\mathrm{min}}(A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}}), 1, \ldots,1, \lambda_{\mathrm{max}}(A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}})\right) $, with 
\begin{eqnarray}
\label{eq:basic2}
\lambda_{\mathrm{min}}(A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}}) &=&  1 + 2 \eta\left(\eta - \alpha - \sqrt{\eta^2 - 1 }\right)  = -1 + 2\eta^2 - 2\eta \sqrt{\eta^2-1}\\
\lambda_{\mathrm{max}}(A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}})&=& 1 + 2\eta \left(\eta - \alpha + \sqrt{\eta^2 -1 }\right) = -1 + 2\eta^2 + 2\eta \sqrt{\eta^2-1} ~.
\end{eqnarray}
In fact, we claim that $|\alpha|<1$ with probability $1$, which by Lemma \ref{lem:basiclem} implies that 
\begin{align}
\label{eq:cuc2}
\lambda_{\mathrm{min}}(A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}})<1<\lambda_{\mathrm{max}}(A_{\varepsilon^{(1)}}^\top A_{\varepsilon^{(1)}})\;. 
\end{align}
Indeed, recalling from Lemma \ref{lem:basiclem} that by definition $\alpha = \inner{\frac{{x}_1}{\|{x}_1\| },\frac{\tilde{x}_1}{\|\tilde{x}_1\| }}$ with $\tilde{x}_1 = (X^\top X)^{-1} x_1$, first observe that $|\alpha|<1$ almost surely. Indeed, $|\alpha|=1$ iff $\tilde{x}_1$ and $x_1$ are colinear, that is for some scalar $\lambda$ it holds $(X^\top X)^{-1} x_1 = \lambda x_1$, which in particular implies that $x_1$ is an eigenvector of $(X^\top X)^{-1}$, or equivalently of $X^\top X$. 
Letting $y_i = x_i^\top x_1$, this means that
\begin{align*}
    \lambda x_1 =(X^\top X)x_1 = \left(\sum_i x_i x_i^\top \right) x_1 = \sum_i x_i y_i \;.
\end{align*}
Since $X$ has rank $d$ almost surely, $\{x_i\}_{i=1\ldots d}$ are linearly independent almost surely, which in turn implies that $y_i = \inner{x_1, x_i} = 0$ for $i \neq 1$ almost surely. This is a $0$-probability event since the $x_i$'s are continuously distributed and independent of each other. 

In what follows to ease notation we denote $\varepsilon^{(1)}$ simply by $\varepsilon$ and in particular $A_{\varepsilon^{(1)}}$ simply by $A_{\varepsilon}$. In the following lemma we establish that $\eta \lesssim d^2$ with probability close to $1$. The proof of this fact is given in Section~\ref{sec:auxiliary}. More precisely, we claim the following:
\begin{lemma}
\label{lem:etabounds}
There exist constants $C>0$ and $d_0 > 0$ such that for any $d \geq d_0$,
\begin{align*}
    \mathbb{P}\left(\eta \leq C d^2 \right) \geq 1 - 1/d\;.
\end{align*}
\end{lemma}
 
We shall now establish (\ref{eq:ITpart1}) building from Lemma \ref{lem:etabounds}. We first relate the spectrum of $A_\varepsilon$ with the probability that $ \| A_\varepsilon {w} \|_2 < \|{w} \|_2$ or equivalently $ \left\| A_\varepsilon \frac{{w}}{\|{w} \|_2} \right\|_2 < 1$. Let $\check{w}:=w/\|w\|$, so 
 ${w} = \gamma \check{w}$, with
 $\check{w} \in {S}^{d-1}$ uniformly distributed, and independent from $\gamma$. 
We claim that with respect to the randomness of $\check{w}$ but conditioning on $X$ it holds \begin{align}
\label{eq:ITlem_rr} 
\mathbb{P}_{\check{w}} ( \| A_\varepsilon \check{w} \| < 1 ) = \frac{2}{\pi} \arcsin\left(\sqrt{\frac{1-\lambda_\mathrm{min}(A_\varepsilon^\top A_\varepsilon)}{\lambda_\mathrm{max}(A_\varepsilon^\top A_\varepsilon)-\lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon)}} \right)~.  
\end{align}
Indeed, assuming without loss of generality that the two eigenvectors of $A_\varepsilon^\top A_\varepsilon$ associated with the distinct eigenvalues $\lambda_{\min}(A_\varepsilon^\top A_\varepsilon)$ and $\lambda_{\max}(A_\varepsilon^\top A_\varepsilon)$ are respectively $e_1$ and $e_2$, the first two standard basis vectors, we have that \begin{align*}\|A_\varepsilon \check{w} \|_2^2 =  \lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \check{w}_1^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \check{w}_2^2 + \sum_{i>2} \check{w}_i^2~,\end{align*}
and therefore, using the uniform distribution on ${S}^{d-1}$ of $\check{w}$, it holds
\begin{eqnarray}
\label{eq:cuc1}
\mathbb{P}_{\check{w}} ( \| A_\varepsilon \check{w} \|_2 < 1 ) &=&  \mathbb{P}_{\check{w}} ( \| A_\varepsilon \check{w} \|_2^2 \leq \|\check{w}\|^2 ) \nonumber \\
&=& \mathbb{P}_{\check{w}} ( \lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \check{w}_1^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \check{w}_2^2 \leq \check{w}_1^2 + \check{w}_2^2 ) \nonumber \\
&=& \mathbb{P}_{\check{w}} \left( \lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \frac{\check{w}_1^2}{\check{w}_1^2 + \check{w}_2^2} + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \frac{\check{w}_2^2}{\check{w}_1^2 + \check{w}_2^2} \leq 1 \right) \nonumber \\
&=& \mathbb{P}_{\theta \sim U[0,2\pi]} \left( \lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \cos(\theta)^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \sin(\theta)^2 \leq 1 \right)~,
\end{eqnarray}
where the last equality follows since the marginal of $\check{w}$ corresponding to the first two coordinates is also rotationally invariant. 

From the last identity of (\ref{eq:cuc1}) and (\ref{eq:cuc2}), we verify that 
\begin{eqnarray*}
 & \mathbb{P}_{\theta \sim U[0,2\pi]}& \left( \lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \cos(\theta)^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \sin(\theta)^2 \leq 1 \right) \\
 &=& \frac{1}{2\pi} \int_{0}^{2\pi} \one\left[\lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \cos(\theta)^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \sin(\theta)^2 \leq 1 \right] d\theta \\
 &=& \frac{2}{\pi} \int_{0}^{\pi/2} \one\left[\lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \cos(\theta)^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \sin(\theta)^2 \leq 1 \right] d\theta \\
 &=& \frac{2}{\pi} \theta^*~,
\end{eqnarray*}
where $\theta^*$ is the only solution in $(0, \pi/2)$ of 
\begin{align}
\label{eq:cuc3}
\lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon) \cos(\theta)^2 + \lambda_{\mathrm{max}}(A_\varepsilon^\top A_\varepsilon) \sin(\theta)^2 = 1~.    
\end{align}
From (\ref{eq:cuc3}) we obtain directly (\ref{eq:ITlem_rr}), as claimed.

Now, the quantity $\rho:=\frac{1-\lambda_\mathrm{min}(A_\varepsilon^\top A_\varepsilon)}{\lambda_\mathrm{max}(A_\varepsilon^\top A_\varepsilon)-\lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon)}$, expressed in terms of $\alpha=1/\eta$ and $\eta$ becomes
\begin{align*}
\rho=\frac{1-\lambda_\mathrm{min}(A_\varepsilon^\top A_\varepsilon)}{\lambda_\mathrm{max}(A_\varepsilon^\top A_\varepsilon)-\lambda_{\mathrm{min}}(A_\varepsilon^\top A_\varepsilon)} =  \frac{-\eta^2 + \eta \sqrt{\eta^2-1}+1}{2\eta \sqrt{\eta^2-1} }~,
\end{align*}
and satisfies $0 \leq \rho=\rho(\eta) < 1$ almost surely.  
Denoting 
\begin{align*}
    f(\eta):= \arcsin \left(\sqrt{\rho} \right)\;,
\end{align*}
we verify that $f'(\eta) < 0$ for $\eta \geq 1$. In order to leverage Lemma \ref{lem:etabounds}, we consider the event that $\eta \leq C_2 d^2$. We can lower bound $f(\eta)$ as follows.
First, observe that $t \mapsto \arcsin(\sqrt{t})$ is non-decreasing in $t\in (0, 1)$, thus 
\begin{align*}
f(\eta) \geq \arcsin\left(\sqrt{\frac{\eta(\sqrt{\eta^2 -1} - \sqrt{\eta^2} ) +1 }{2\eta^2}}\right)\;,
\end{align*}
since 
\begin{align*}
    \frac{-\eta^2 + \eta \sqrt{\eta^2-1}+1}{2\eta \sqrt{\eta^2-1} } \geq  \frac{-\eta^2 + \eta \sqrt{\eta^2-1}+1}{2\eta^2 }= \frac{\eta(\sqrt{\eta^2 -1} - \sqrt{\eta^2} ) +1 }{2\eta^2}\;.
\end{align*}
Moreover, since $\sqrt{t+1} - \sqrt{t} = \frac{1}{2\sqrt{t}} + O(t^{-3/2})$, we have that 
\begin{align*}
\frac{\eta(\sqrt{\eta^2 -1} - \sqrt{\eta^2} ) +1 }{2\eta^2} = \frac{3}{4}\eta^{-2} + O(\eta^{-4})\;,
\end{align*}
which, combined with the fact that $\arcsin(t) = t + O(t^3)$ for $|t| \le 1$, leads to 
\begin{align*}
    f(\eta) \geq \frac{3}{4}\eta^{-1} + O(\eta^{-2})\;.
\end{align*}
Finally, using Lemma \ref{lem:etabounds} and the definition of $f(\eta)$, we obtain that 
\begin{align*}
    \mathbb{P}_{\check{w}}(\| A_\varepsilon \check{w} \| \leq 1 ) \geq \frac{6}{4\pi C_2}d^{-2} + O(d^{-4})    
\end{align*}
with probability (over $X$) greater than $1/2$.
Since $X$ and $w$ are independent, we conclude that
\begin{align}
\label{eq:ITlem_r1}
    \mathbb{P}_{X,\check{w}}(\| A_\varepsilon \check{w} \| \leq 1 ) \geq \frac{1}{2} \left(\frac{6}{4\pi C_2}d^{-2} + O(d^{-4})\right)= C_4 d^{-2} + O(d^{-4})~~,
\end{align}
where $C_4$ is a constant.

Now we show that 
\begin{align*}
\mathbb{P}_{\check{w}} \left(\| A_\varepsilon \check{w} \|_2^2 \geq 1 - 1/\sqrt{d}\right) \geq 1-\exp\left(-\Omega(\sqrt{d})\right) \;.
\end{align*}
Recall that $\check{w}$ is distributed uniformly on the sphere $S^{d-1}$, and that all eigenvalues of $A_{\varepsilon}^{\top} A_{\varepsilon}$ are all greater or equal to 1, except for $\lambda_\mathrm{min}$. Assuming without loss of generality that $e_1$ is the eigenvector corresponding to $\lambda_{\mathrm{min}}$, we have for any $\check{w} \in S^{d-1}$,
\begin{align*}
    \|A_\varepsilon \check{w}\|_2^2 \ge 1-\check{w}_1^2\;.
\end{align*}
Let $H$ be the hemisphere $H=\{\check{w}_1 \le 0 \mid \check{w} \in S^{d-1}\}$. By the classic isoperimetric inequality for the unit sphere $S^{d-1}$~\cite[Chapter 1]{ledoux2001concentration}, the measure of the $r$-neighborhood of $H$, which we denote by $H_r = \{u \in S^{d-1} \mid \mathrm{dist}(u,H) \le r\}$, satisfies
\begin{align*}
    \mathbb{P}_{\check{w}}(H_r) = \mathbb{P}_{\check{w}}(\check{w}_1 \le r) \ge 1-\exp(-(d-1)r^2/2)\;.
\end{align*}
An analogous inequality holds for the event $\{\check{w}_1 \ge -r\}$ by the sign symmetry of the distribution of $\check{w}$. Plugging in $r=d^{-1/4}$, It follows that
\begin{align*}
\mathbb{P}_{\check{w}} \left(\| A_\varepsilon \check{w} \|^2 \geq 1 - 1/\sqrt{d}\right) 
&\geq \mathbb{P}_{\check{w}} \left(1-\check{w}_1^2 \geq 1 - 1/\sqrt{d}\right) \\
&= \mathbb{P}_{\check{w}} \left(|\check{w}_1| \le 1/d^{1/4}\right) \\
&\geq 1-\exp\left(-\Omega(\sqrt{d})\right)\;.
\end{align*}

Therefore, combining the above with (\ref{eq:ITlem_r1}) using the union bound, we obtain
\begin{align}
\label{eq:ITlem66}
    \mathbb{P}_{X,\check{w} }\left(\sqrt{1 -  d^{-1/2}} \leq \| A_\varepsilon {\check{w}} \| \leq 1  \right) \geq C_4 d^{-2} + O(d^{-4}) - \exp(-\Omega(\sqrt{d})) = C_4 d^{-2} + O(d^{-4}) ~.
\end{align}
Finally, since $B>\sqrt{2}$ and $\sqrt{1-d^{-1/2}} \ge 1/\sqrt{2}$, we have 
\begin{align}
\label{eq:ITlem67}
\mathbb{P}_{\tilde{w}}( \gamma \sqrt{1 -  d^{-1/2}} \geq 1 ) &=& \mathbb{P}_{\tilde{w}}\left( \gamma \geq \frac{1}{\sqrt{1 -  d^{-1/2}}} \right) \nonumber \\ 
&=& \int_{\frac{1}{\sqrt{1 -  d^{-1/2}}}}^B {q_\gamma}(v) dv := Q_s
\end{align}

Since ${w} = \gamma \check{w}$, where $\check{w}$ is uniformly distributed in $\mathcal{S}^{d-1}$ and $\gamma$ is independent of $\check{w}$, we conclude by assembling (\ref{eq:ITlem66}) and (\ref{eq:ITlem67}) that

\begin{align*}
    \mathbb{P}_{X,{w}} \left(1 \leq \| A_\varepsilon {w} \| \leq \|{w}\|  \right) \geq (C_4 d^{-2} + O(d^{-4})) Q_s = C_5 d^{-2} + O(d^{-4})~,
\end{align*}
since $Q_s \geq Q_{1/\sqrt{2}} \geq C$ 
for $d\geq 2$ thanks to Assumption \ref{assump:basic}. This concludes the proof of (\ref{eq:ITpart1}).
\end{proof}


\subsection{Auxiliary Lemmas}
\label{sec:auxiliary}

\begin{proof}[Proof of Lemma \ref{lem:mapoptim}]
Observe that
\begin{align*}
    \mathbb{P}( \hat{x} \neq x^*) = 1- \mathbb{P}(\hat{x} = x^*) = 1 - p(\hat{x} | y) \geq 1 - \max_x p( x| y)\;,
\end{align*}
with equality if $\hat{x}$ is the Maximum-a-Posteriori estimator. 
\end{proof}


\begin{proof}[Proof of Lemma \ref{lem:basiclem}]
First notice that we can reduce to a two-by-two matrix, since the directions orthogonal to both $u$ and $v$ clearly belong to an eigenspace of eigenvalue $1$. 
The result follows directly by computing the characteristic equation $\det[ A^\top A - \lambda I] = 0$.
\end{proof}



\begin{proof}[Proof of Lemma \ref{lem:etabounds}]
First, observe that since the law of $X$ is rotationally invariant, we can 
assume without loss of generality that $x_1$ is proportional to $e_1^\top$, the first standard basis vector. Using the Schur complement, we have
\begin{align}
\label{eq:simpler}
X = \begin{pmatrix} 
\|x_1\|_2 & 0 \\
v & \bar{X} 
\end{pmatrix}~,\text{ and }~ X^{-1} = \begin{pmatrix} 
\|x_1\|_2^{-1} & 0 \\
b & \bar{X}^{-1} 
\end{pmatrix}~,
\end{align}
where $v$ is the $(d-1)$-dimensional vector given by $v_i = \|x_1\|_2^{-1} \inner{x_1, x_{i+1}} = x_{i+1,1} \sim N(0, 1)$, $\bar{X}$ is a $(d-1) \times (d-1)$ matrix whose entries are drawn i.i.d. from
$N(0,1)$, and $b = - \|x_1\|_2^{-1} \bar{X}^{-1} v$. 
Observe that $\bar{X}$ and $v$ are independent, since the choice of basis depends only on $x_1$. The coordinates of $v$ are independent as well for the same reason.
It follows that
\begin{align}
\label{eq:basicschur}
\| \tilde{x}_1 \|_2^2 
&= \|x_1\|_2^{-2}\left(1 + \| \bar{X}^{-1} v\|_2^2\right)  \nonumber \\
&\le \|x_1\|_2^{-2}\left(1 + \|\bar{X}^{-1}\|^2\cdot \|v\|_2^2\right)\;, 
\end{align}
where $\|\bar{X}^{-1}\| = \max_{u \in S^{d-1}} \|\bar{X}^{-1}u\|_2$ is the operator norm of $\bar{X}^{-1}$. 
Now let $\alpha$ be a fixed constant, which will be specified later. Additionally, assume that $d$ is sufficiently large so that $\alpha d^4 \ge 2$. From Eq.~\eqref{eq:basicschur}, we have that 
\begin{align}
\mathbb{P}\{ \eta^2 \ge \alpha d^4\} 
&\leq \mathbb{P}\left\{  \|x_1\|_2^2 \left( \|x_1\|_2^{-2}\left(1 + \|\bar{X}^{-1}\|^2\cdot \|v\|_2^2\right)  \right) \ge \alpha d^4  \right\} \nonumber \\
&= \mathbb{P} \left\{    1+ \|\bar{X}^{-1}\|^2\cdot\|v\|_2^2  \ge \alpha d^4 \right\} \nonumber \\
&\le \mathbb{P} \left\{    \|\bar{X}^{-1}\|^2\cdot\|v\|_2^2  \ge \alpha d^4/2 \right\} \nonumber \\
&= \mathbb{P} \left\{    \|\bar{X}^{-1}\|\cdot\|v\|_2  \ge \sqrt{\alpha/2}\cdot d^2 \right\} \label{eq:inverse-norm-split-case} \;.
\end{align}
To upper bound Eq.~\eqref{eq:inverse-norm-split-case}, we use the fact that $\bar{X}^{-1}$ and $v$ are independent, and split the event into two cases: $\{\|v\|_2 \ge \sqrt{d}/2\}$ and $\{\|v\|_2 < \sqrt{d}/2\}$. By~\cite[Theorem 3.1.1]{vershynin2018high}, we know that there exists a constant $C_1 > 0$ such that
\begin{align*}
    \mathbb{P}\left\{\|v\|_2 < \sqrt{d}/2\right\} \le \exp(-C_1 \cdot d)\;.
\end{align*}
Moreover, by~\cite[Theorem 1.2]{szarek1991condition}, we have that for sufficiently large $d$, there exists a universal constant $C_2 > 0$ such that for any $t > 0$,
\begin{align*}
    \mathbb{P}\left\{ \|\bar{X}^{-1}\| \ge t \sqrt{d} \right\} \leq C_2/t\;.
\end{align*}
By setting $\alpha = 2C_2^2$ and $d$ sufficiently large so that $\exp(-C_1 d) \le 1/(2d)$, we have
\begin{align}
\mathbb{P} \Big\{    \|\bar{X}^{-1}\|\cdot\|v\|_2  &\ge \sqrt{\alpha/2}\cdot d^2 \Big\} \nonumber \\
&\le \mathbb{P} \left\{    \|\bar{X}^{-1}\|\cdot\sqrt{d}/2  \ge \sqrt{\alpha/2}\cdot d^2 \right\} 
\cdot \mathbb{P} \left\{\|v\|_2 > \sqrt{d}/2\right\} + \mathbb{P}\left\{\|v\|_2 \le \sqrt{d}/2\right\} \nonumber \\
&\le \mathbb{P} \left\{    \|\bar{X}^{-1}\|\cdot\sqrt{d}/2  \ge \sqrt{\alpha/2}\cdot d^2 \right\} + \exp(-C_1 d) \nonumber \\
&= \mathbb{P} \left\{    \|\bar{X}^{-1}\|  \ge \sqrt{2\alpha}\cdot d^{3/2} \right\} + \exp(-C_1 d) \nonumber \\
&\le C_2/(\sqrt{2\alpha} \cdot d) + \exp(-C_1 d) \nonumber \\
&\le 1/d \nonumber \;.
\end{align}
Therefore,
\begin{align*}
\mathbb{P}\{ \eta \ge \sqrt{2}C_2 \cdot d^2\} = \mathbb{P}\{ \eta^2 \ge 2C_2^2 \cdot d^4\} \le \mathbb{P} \Big\{    \|\bar{X}^{-1}\|\cdot\|v\|_2  \ge C_2\cdot d^2 \Big\} \le 1/d \;.
\end{align*}
\end{proof}


